Improving Transformers with Probabilistic Attention Keys

Multi-head attention is a driving force behind state-of-the-art transformers, which achieve remarkable performance across a variety of natural language processing (NLP) and computer vision tasks. It has been observed that for many applications, those attention heads learn redundant embedding, and most of them can be removed without degrading the performance of the model. Inspired by this observation, we propose Transformer with a Mixture of Gaussian Keys (Transformer-MGK), a novel transformer architecture that replaces redundant heads in transformers with a mixture of keys at each head. These mixtures of keys follow a Gaussian mixture model and allow each attention head to focus on different parts of the input sequence efficiently. Compared to its conventional transformer counterpart, Transformer-MGK accelerates training and inference, has fewer parameters, and requires fewer FLOPs to compute while achieving comparable or better accuracy across tasks. Transformer-MGK can also be easily extended to use with linear attention. We empirically demonstrate the advantage of Transformer-MGK in a range of practical applications, including language modeling and tasks that involve very long sequences. On the Wikitext-103 and Long Range Arena benchmark, Transformer-MGKs with 4 heads attain comparable or better performance to the baseline transformers with 8 heads.

==> icml2022/sections/rebuttal.tex <==
\subsection{Review of Reviewer 1}
\textbf{Comment: }The idea is interesting, and the results are compelling with large compute savings. But there are also obvious downsides of this paper, including aforementioned lacking analysis of GMM approximation, saturating effect with enough number of heads, and similarity to another GMM-based transformer paper.

\textbf{Authors' response:} Thank you for your thoughtful review and valuable feedback. Below we address your concerns.

\textbf{Question 1: }I have a few concerns about the GMM approximation in the paper:
\begin{itemize}
    \item First off, how well it approximates the probability distribution of attention in practice? Any empirical observation from experiments?
    
    \textbf{Authors' Answer:} One way to approximate the probability distribution of attention in practice is to compute the negative likelihood (NLL) score of our MGK. The smaller the negative likelihood, the better MGK fits the distribution of the queries and the attention. We have computed the NLL of the MGK in comparison with the NLL of the baseline model that uses only 1 Gaussian distribution centered around the key $k_j$ at each time j. We observed that the NLL of the MGK is xxxx which is smaller than the NLL xxxx of the baseline.
    
    \item Are the learned GMMs diverse enough? Fig.~\ref{fig:attention-viz} only visualizes the final attention scores, but not different Gaussians in each head.
    
    \textbf{Authors' Answer:} We believe there is a misunderstanding of our results in Fig. 2. Please allow us to clear this misunderstanding. In MGK, we replace the key $k_j$ by a mixture of keys and then compute an attention matrix at each head whose elements, i.e. attention scores, are given by Eqn. (7) in our manuscript. Thus, in Transformer-MGK, there is only one attention matrix at each head which we plot in Fig.~\ref{fig:attention-viz} (Left). From Fig.~\ref{fig:attention-viz} (Left), we observe that these attention matrices have more diverse patterns than those in the baseline softmax transformers, which prove the learned GMM is more diverse than the single Gaussian distribution in the baseline. This observation is further confirmed in Fig.~\ref{fig:attention-viz} (Right) which shows that average rank distribution of attention matrices in Transformer-MGK is higher than in the baseline.
    
    \item Along this line, setting M=2 with fixed variance (so only Gaussian means are learned, as mentioned in L206-L208) should further hurt the diversity and expressiveness of GMMs. Any ablations on these design choices?
    
    \textbf{Authors' Answer:} In our experiments, we set M=2 and $\sigma^{2}_{j1}$ = $\sqrt(D)$ as in the baseline softmax transformer and $\sigma^{2}_{j2}$ = $3\sqrt(D)$ where $D$ is feature dimension defined in Section 1.1 of our manuscript. As you suggested, we have conducted an ablation study on the IWSLT14 De-En machine translation task in which we vary  $\sigma^{2}_{j2}$ among the following values, $\sigma^{2}_{j2}$ = $0.5\sqrt(D), \sqrt(D), 2\sqrt(D), 3\sqrt(D), 4\sqrt(D)$. We observe that the BLEU score of the trained models do not differ much between different values of $\sigma^{2}_{j2}$. We also make $\sigma^{2}_{j1}$ and $\sigma^{2}_{j2}$ learnable and observe the same result that the BLEU score of the trained models is not much different from fixing these variances. We report our ablation study results in the Table~\ref{tab:2nd_D}.
    
\end{itemize}

\begin{table}[t!]
\small
    \caption{\small BLUE scores of Transformer-MGK on the IWSLT14 De-En machine translation task as $\sigma^{2}_{j2}$ is varied: $\sigma^{2}_{j2}$ = $\alpha*\sqrt(D)$, with $\alpha \in \{0.5, 1, 2, 3, 4\}$}
    \vspace{-0.5em}
    \begin{center}
    \scalebox{0.9}{
    \begin{tabular}{lc}
    \toprule
        $\alpha$ & BLEU \\
        \midrule
        0.5 & 34.31 \\
        1 & 34.36 \\
        2 & 34.61 \\
        3 & 34.34 \\
        4 & 34.27 \\
        \textcolor{blue}{Learnable  & 32.86}
        
        \bottomrule
    \end{tabular}}
    \end{center}
\vspace{-0.5em}
\label{tab:2nd_D}
\end{table}

\textbf{Question 2: }Another question is about the query/key normalization that may impact the approximation capability of GMM. As mentioned under Eq (6): the assumption that the queries and keys are normalized is relaxed, and the Gaussian kernels between queries and keys instead are directly computed. Will this un-normalized L2 approximation result in training instability or other degradation?

\textbf{Authors' Answer: }As proven in [1], the normalized attention where the queries and keys are normalized as in the baseline transformer is not Lipschitz. The un-normalized L2 approximation that we use is  Lipschitz (see Section 3.2 and Theorem 3.2 in [1]). This Lipschitz property of un-normalized L2 self-attention helps stabilize training and endows models with provable robustness and guaranteed generalization bound [1].

\textbf{Question 3: }The required EM step actually imposes some changes to the training paradigm, and concrete complexity analysis is missing.

\textbf{Authors' Answer: }In Fig.~\ref{fig:speed_param_compare_update_method} in the supplementary, we present an empirical complexity analysis for different EM-based inference and learning methods for Transformer-MGKs trained on the document and retrieval task. We observe that the computational costs in terms of FLOPS and model size in terms of the number of parameters are almost the same between these methods. Note that in Fig. 8, Transformer-MGK is the default model that we use in all of our experiments where the soft E-step is used, the mixing coefficients $\pi_{jr}$ and the key $k_{jr}$ are learnable via SGD, and the variance $\sigma^{2}_{jr}$ are constants. Transformer-MGK Hard-E is the Transformer-MGK where the hard E-step is used, the mixing coefficients $\pi_{jr}$ and the key $k_{jr}$ are learnable via SGD, and the variance $\sigma^{2}_{jr}$ are constants. Transformer-MGK Soft-E is the Transformer-MGK where the soft E-step is used, the mixing coefficients $\pi_{jr}$ are updated according to the M-step update in, the key $k_{jr}$ are learnable via SGD, and the variance $\sigma^{2}_{jr}$ are constants. Transformer sMGK is the Transformer MGK with shifted keys as explained in “Design Options for Keys” in Section 2.3 of our manuscript. 

In addition, a complexity analysis with detailed formulas of the default Transformer-MGK in comparison with the baseline softmax transformer is given in Appendix~\ref{sec:compt-params-analysis}

\textbf{Question 4: }The whole set of experiments are conducted in a way that proves Transformer-MGK/MLK can use only half the number of attention heads to achieve comparable performance with standard Transformer. Then one question naturally arises: will Transformer-MGK/MLK drastically improve performance with the same number of heads? Table 3 seems to give a negative answer to that. (s)MGK 8 heads give marginal gains over Softmax 8 heads, much smaller than the gap between MGK 4 heads and Softmax 4 heads. Does it mean saturating effect of MGK/MLK given enough number of heads? More experiments are needed here.

\textbf{Authors' Answer: }When using more heads, the improvement in accuracy of MGK using the same number of heads over the baseline softmax/linear transformer is smaller. This is because the baseline model has already obtained good accuracy given its capacity. To further improve its accuracy is challenging, and that MGK/MLK manages to improve the accuracy of the baseline model in this case demonstrates the advantage of our methods. Also,  in our work, we focus on using MGK to increase the efficiency of the baseline softmax/linear transformers models, thus a better use case of MGK for the WikiText-103 language modeling experiments presented in Table~\ref{tab:lm-results} is to replace a 8-head softmax/linear transformers with a 4-head MGK/MLK for comparable or even better accuracy with much better efficiency.



\textbf{Question 5: }The GMM approximation lacks some analysis and bears similarities to existing literature. The following paper is closely related in that it applies GMM to improve cross-attention. I think it's worth some discussions and comparisons.

\textbf{Authors' Response: }


\subsection{Review of Reviewer 4}

\textbf{Authors' Response: }Thank you for your thoughtful review and valuable feedback. Below we address your concerns.

\textbf{Question 1: }The improvement over linear transformer seems marginal. The results in Table 2 is mixed. It may not be convincing enough that Transformer-MLK is a stronger alternative to linear Transformers.

\textbf{Authors' Answer: }We believe there is a misunderstanding of our results in Table~\ref{tab:LRA_linear} that together with Fig.~\ref{fig:flops_params} show the advantage of Transformer-MLK over the baseline linear transformers. Please allow us to clear this misunderstanding. In Table~\ref{tab:LRA_linear}, we show that the Transformer-MLK/Transformer-sMLK with only 2 and 4 heads obtain better results than the baseline linear transformer with 4 and 8 heads in the ListOps and document retrieval task while achieving comparable results with the baselines in the text classification task. Averaging the results over these three tasks, our Transformer-MLK/Transformer-sMLK obtains better results than the baseline. On another hand, in Fig.~\ref{fig:flops_params}, we show that the Transformer-MLK is much more efficient than baseline linear transformers in terms of FLOPs and the number of parameters. Note that, similar to the results for Transformer-sMGK and Transformer-MGK, Transformer-sMLK has similar computational cost in terms of FLOPS  as Transformer-MLK but with fewer parameters. The efficiency advantage of Transformer-MLK over the baseline linear transformers is also shown in Fig.~\ref{fig:lm_efficiency_linear} and Table~\ref{tab:time_memory_retrieval}. The advantage in terms of accuracy of Transformer-MLK over the baseline linear transformers is also shown in Table~\ref{tab:12_head_retrieval}

\subsection{Review of Reviewer 5}

\textbf{Authors' Response: }Thank you for your thoughtful review and valuable feedback. Below we address your concerns.

\textbf{Question 1: }How hard would it for this to be implemented? It does seem that there's a lot going on especially with the usage of the EM algorithm. If this is like a couple lines change in a transformer i could see this getting adoption, but no one is going to implement so much just for this.

\textbf{Authors' Answer: }It is very easy and straightforward to implement our MGK and MLK methods. We have included our code in the supplementary material, and you can see how simple it is to implement MGK and MLK in our submitted code. For example, for the WikiText-103 task, the MGK and MLK are implemented in the class MGKAttn and CudaFastWeightSumTwoLinearTransformerLayer in language-modeling/lmtool-fwms/src/mem\_transformer.py, respectively.

\subsection{Review of Reviewer 6}

\textbf{Authors' Response: }Thank you for your thoughtful review and valuable feedback. Below we address your concerns.

\textbf{Question 1: }Although it is nice to save parameters, recent works suggest the problem is less urgent as sparse models do work well e.g. ~\cite{https://doi.org/10.48550/arxiv.2112.06905}. After all, most deep models are overparameterized but still work well empirically.

\textbf{Authors' Answer: }The efficiency advantage of our MGK/MLK is not only saving parameters but also to reducing the computational costs in terms of FLOPs and computational overhead (seconds/iteration) (see Fig.~\ref{fig:lm_flops_params},~\ref{fig:flops_params},~\ref{fig:lm_efficiency_linear} and Table 7) and saving the memory usage (see Table~\ref{tab:time_memory_retrieval}). These advantages are important at inference time for the model deployment. Our method is complementary to sparse models like GLaM~\cite{https://doi.org/10.48550/arxiv.2112.06905} in and can be used with sparse models to further improve the efficiency of transformers.

\textbf{Question 2: }Experiments are done mostly on small scales in terms of model sizes and datasets. Numbers seem to be far away from current art and gains are not so clear in some cases. For example, the BLEU scores in table 4 probably won't be statistically significant enough.

\textbf{Authors' Answer: }Our experiments to show the advantage of MGK/MLK cover large-scale tasks including the WikiText-103 language modeling, which is popularly used to validate the performance of new proposed transformers. On this task, in addition to the small baseline transformer, we also provide empirical results for the MGK/MLK applied on the medium baseline transformer. This model has 90M parameters, 16 layers, 8 attention heads per layer, and hidden size of 256. The size of our baseline model is close to BERTBase~\cite{https://doi.org/10.48550/arxiv.1810.04805}, which has 110M parameters, 12 layers, 12 attention heads per layer, and hidden size of 768. Note that the baseline transformer we used is deeper than BERTBase. This baseline transformer attains a test perplexity (PPL) of 29.60 as reported in~\cite{schlag2021linear}, which, on this WikiText-103 task, is better than or equivalent to popular transformer models including~\cite{https://doi.org/10.48550/arxiv.1612.04426},~\cite{article},~\cite{merityAnalysis},~\cite{pmlr-v80-rae18a}, and~\cite{shaw-etal-2018-self}.  Applying our MGK on top of this new larger baseline, we significantly improve the test PPL to 28.86.

To further examine the scalability of our method, we compare the 8-head Transformer-MGK/sMGK with the 16-head Softmax Transformer on the WMT' 14 machine translation task. The 16-head baseline consists 12 layers, i.e., 6 encoder and 6 decoder layers with 201M trainable parameters. The 8-head transformer-MGK and sMGK have the same configuration as the baseline except for the number of heads at each layer. In this task, Transformer-MGK and Transformer-sMGK obtain the BLEU score of 29.03 and 29.07, respectively, which are both better than the BLEU score of 29.38 of the 16-head baseline softmax transformer.

